Higher-Order Constrained Horn Clauses and Refinement Types

Motivated by applications in automated verification of higher-order functional programs, we develop a notion of constrained Horn clauses in higher-order logic and a decision problem concerning their satisfiability. We show that, although satisfiable systems of higher-order clauses do not generally have least models, there is a notion of canonical model obtained through a reduction to a problem concerning a kind of monotone logic program. Following work in higher-order program verification, we develop a refinement type system in order to reason about and automate the search for models. This provides a sound but incomplete method for solving the decision problem. Finally, we show that an extension of the decision problem in which refinement types are used directly as guards on existential quantifiers can be reduced to the original problem. This result can be used to show that properties of higher-order functions that are definable using refinement types are also expressible using higher-order constrained Horn clauses.

==> apx-mono-models.tex <==
%

\section{Proofs from Section 4}

\begin{lemn}[\ref{lem:models-pfps}]
For definite formula $\Delta \sorts D : o$, the prefixed points of $\sfunc_{(P_D:\Delta)}$ are exactly the models of $D$.
\end{lemn}
\begin{proof}
We assume without loss of generality that $D$ has the shape specified in the above exposition.
%
%
%
%

In the forward direction, assume that, for all $i \in 1..\ell$, $\smng{\forall \vv{x_{r_i}}.\,s_i \implies \term{X_{r_i} \vv{x_{r_i}}}}(\alpha)$.
Then, for each $j \in 1..k$, $\sfunc_{P_D:\Delta}(\alpha)(X_j) = \smng{\abs{\vv{x_j}}{G_j'}}(\alpha)$.
Let $\vv{t}$ be such that $\smng{\abs{\vv{x_j}}{G_j'}}(\alpha)\,\vv{t} = 1$.
Then it follows that $\smng{G_j'}(\alpha[\vv{x_j} \mapsto \vv{t}]) = 1$.
By definition, then, there is some $i \in 1..\ell$ such that $r_i = j$ and $\smng{G_i}(\alpha[\vv{x_j} \mapsto \vv{t}]) = 1$.
Therefore, it follows from the assumption that $\smng{\term{X_j \vv{x_j}}}(\alpha[\vv{x_j}\mapsto\vv{t}]) = 1$, i.e. $\smng{X_j}(\alpha)\,\vv{t} = 1$.
Since $\vv{t}$ was arbitrary, it follows that $\smng{\abs{\vv{x_j}}{G_j}}(\alpha) \subseteq \smng{X_j}(\alpha) = \alpha(X_j)$.
Since $j$ was arbitrary, it follows that $\alpha$ is a prefixed point of $\sfunc_{P_D:\Delta}$.

In the backward direction, assume that $\alpha$ is a prefixed point of $\sfunc_{P_D:\Delta}$.
That is, for all $j \in 1..k$, $\smng{\abs{\vv{x_j}}{G_j'}}(\alpha) \subseteq \smng{X_j}(\alpha)$.
Let $i \in 1..\ell$ and let $\vv{t}$ be an appropriate vector of values for $\vv{x_{r_i}}$.
Then assume $\smng{G_i}(\alpha[\vv{x_{r_i}}\mapsto\vv{t}]) = 1$.
By construction, there is some $j \in 1..k$ such that $r_i = j$, so it follows that $\smng{G_j'}(\alpha[\vv{x_j}\mapsto\vv{t}]) = 1$, since $G_i$ is one of the disjuncts.
Consequently, $\smng{\abs{\vv{x_j}}{G_j'}}(\alpha)\,\vv{t} = 1$ follows by definition.
Hence, it follows from the assumption that $\smng{X_j}(\alpha)\,\vv{t} = 1$.
By definition, this is the same as $\smng{\term{X_j \vv{x_j}}}(\alpha[\vv{x_j}\mapsto\vv{t}])$ as required.
\end{proof}

\begin{lemma}\label{lem:galois-relations}
Fix relational sort $\rho$.  The mappings $\iembed_{\rho}$, $\lomon_\rho$, $\upmon_\rho$ and $\jembed_\rho$ are monotone mappings between the posets prescribed in the above diagram.  Furthermore:
\begin{enumerate}[(i)]
\item For all $s \in \smng{\rho}$, $\jembed_\rho(\upmon_\rho(s)) \subseteq s$.
\item For all $r \in \mmng{\rho}$, $\upmon_\rho(\jembed_\rho(r)) = r$.
\item For all $s \in \smng{\rho}$, $s \subseteq \iembed_\rho(\lomon_\rho(s))$.
\item For all $r \in \mmng{\rho}$, $r = \lomon_\rho(\iembed_\rho(r))$.
\end{enumerate}
\end{lemma}
\begin{proof}
We first prove the initial claim, i.e for all $\rho$:
\begin{enumerate}[(a)]
  \item For all $s \in \smng{\rho}$, $\upmon_{\rho}(s) \in \mmng{\rho}$
  \item For all $r \in \mmng{\rho}$, $\iembed_{\rho}(r) \in \smng{\rho}$
  \item For all $s \in \smng{\rho}$, $\lomon_{\rho}(s) \in \mmng{\rho}$
  \item For all $r \in \mmng{\rho}$, $\jembed_{\rho}(r) \in \smng{\rho}$
  \item For all $s_1, s_2 \in \smng{\rho}$, $s_1 \subseteq s_2$ implies \changed[tcb]{	$\upmon_\rho(s_1) \subseteq \upmon_{\rho}(s_2)$}.
  \item For all $r_1, r_2 \in \mmng{\rho}$, $r_1 \subseteq r_2$ implies $\iembed_\rho(r_1) \subseteq \iembed_{\rho}(r_2)$.
  \item For all $s_1, s_2 \in \smng{\rho}$, $s_1 \subseteq s_2$ implies \changed[tcb]	{$\lomon_\rho(s_1) \subseteq \lomon_{\rho}(s_2)$}.
  \item For all $r_1, r_2 \in \mmng{\rho}$, $r_1 \subseteq r_2$ implies $\jembed_\rho(r_1) \subseteq \jembed_{\rho}(r_2)$.
\end{enumerate}
We proceed by induction on $\rho$.
\begin{itemize}
  \item When $\rho$ is $\boolsort$, all of the claims follow immediately.
  \item When $\rho$ is $\iota \to \rho'$, all of the claims follow immediately from the induction hypothesis, the fact that all functions on the discrete posets $\smng{\iota}$ and $\mmng{\iota}$ are monotone and the fact that composition preserves monotonicity.
  \item When $\rho$ is of shape $\rho_1 \to \rho_2$ we examine the cases as follows.  Claims (b), (d), (f) and (h) follow as in the previous case.
  \begin{itemize}
    \item To see (a), let $r_1, r_2 \in \mmng{\rho_1}$ such that $r_1 \subseteq r_2$.  Then $\upmon_\rho(s)(r_1) = \bigcap\{\upmon_{\rho_2}(s(t)) \mid \iembed_{\rho_2}(r_1) \subseteq t\}$.  It follows from the induction hypothesis that $\iembed_{\rho_2}(r_1)$ is monotone, so $\iembed_{\rho_1}(r_1) \subseteq \iembed_{\rho_1}(r_2)$ and consequently $\{\upmon_{\rho_2}(s(t)) \mid \iembed_{\rho_2}(r_1) \subseteq t\} \supseteq \{\upmon_{\rho_2}(s(t)) \mid \iembed_{\rho_2}(r_2) \subseteq t\}$.  The result follows immediately.
    \item To see (c), let $r_1, r_2 \in \mmng{\rho_1}$ such that $r_1 \subseteq r_2$.  Then $\lomon_{\rho}(s)(r_1) = \bigcup\{\lomon_{\rho_2}(s(t)) \mid t \subseteq \jembed_{\rho_1}(r_1)\}$.  It follows from the induction hypothesis that $\jembed_{\rho_1}$ is monotone, so $\jembed_{\rho_1}(r_1) \subseteq \jembed_{\rho_1}(r_2)$.  Hence $\{\lomon_{\rho_2}(s(t)) \mid t \subseteq \jembed_{\rho_1}(r_1) \} \subseteq \{\lomon_{\rho_2}(s(t)) \mid t \subseteq \jembed_{\rho_1}(r_2) \}$.  The result follows immediately.
    \item To see (e), let $s_1,s_2 \in \smng{\rho}$ with $s_1 \subseteq s_2$.  $\upmon_\rho(s_i)(r) = \bigcap\{\upmon_{\rho_2}(s_i(t)) \mid \iembed_{\rho_2}(r) \subseteq t\}$.  Since, for all $t$, $s_1(t) \subseteq s_2(t)$, it follows from the induction hypothesis that $\upmon_{\rho_2}(s_i)(r) \subseteq \upmon_{\rho_2}(s_i)(r)$.  Hence, we can conclude the desired result.
    \item To see (h), let $s_1,s_2 \in \smng{\rho}$ with $s_1 \subseteq s_2$.  $\lomon_\rho(s_i)(r) = \bigcup\{\lomon_{\rho_2}(s_i(t)) \mid t \subseteq \iembed_{\rho_2}(r)\}$.  Since, for all $t$, $s_1(t) \subseteq s_2(t)$, it follows that $\lomon_{\rho_2}(s_i)(r) \subseteq \lomon_{\rho_2}\rho(s_i)(r)$.  Hence, we can conclude the desired result.
  \end{itemize}
\end{itemize}
Next we prove each of (i) to (iv) by induction on $\rho$.  When $\rho$ is $\boolsort$ the claims follow immediately.  When $\rho$ is of shape $\iota \to \rho'$, the claims follow immediately from the induction hypothesis in each case.  When $\rho$ is of shape $\rho_1 \to \rho_2$, we proceed as follows.
\begin{enumerate}[(i)]
  \item Assume $s \in \smng{\rho}$, then:
  \[
    \begin{array}{rl}
    & \jembed_{\rho}(\upmon_{\rho}(s))(r) \\
    =& \jembed_{\rho_2}(\upmon_{\rho}(s)(\upmon_{\rho_1}(r))) \\
    =& \jembed_{\rho_2}(\bigcap\{\upmon_{\rho_2}(s(t)) \mid \jembed_{\rho_1}(\upmon_{\rho_1}(r)) \subseteq t\}) \\
    \subseteq&  \bigcap\{\jembed_{\rho_2}(\upmon_{\rho_2}(s(t))) \mid \jembed_{\rho_1}(\upmon_{\rho_1}(r)) \subseteq t\})
    \end{array}
  \]
  Since it follows from part (h) that $\jembed_{\rho_2}$ is monotone.  It follows from the induction hypothesis that $\jembed_{\rho_1}(\upmon_{\rho_1}(r)) \subseteq r$, so $\jembed_{\rho_2}(\upmon_{\rho_2}(s(r)))$ belongs to the given set comprehension, whence $\jembed_{\rho_2}(\upmon_{\rho_2}(s(r)))$ is an upper bound on the meet.  It follows from the induction hypothesis that $\jembed_{\rho_2}(\upmon_{\rho_2}(s(r)))$ is itself bounded above by $s(r)$, as required.

  \item Assume $r \in \mmng{\rho}$, then:
  \[
    \begin{array}{rl}
    & \upmon_\rho(\jembed_{\rho}(r))(s) \\
    =& \bigcap\{\upmon_{\rho_2}(\jembed_{\rho}(r)(t)) \mid \jembed_{\rho_1}(s) \subseteq t\} \\
    =& \bigcap\{\upmon_{\rho_2}(\jembed_{\rho_2}(r(\upmon_{\rho_1}(t)))) \mid \jembed_{\rho_1}(s) \subseteq t\} \\
    \end{array}
  \]
  It then follows from the induction hypothesis that\\ $\upmon_{\rho_2}(\jembed_{\rho_2}(r(\upmon_{\rho_1}(t)))) = r(\upmon_{\rho_1}(t))$.  Since $r$ is monotone, $\{r(\upmon_{\rho_1}(t)) \mid \jembed_{\rho_1}(s) \subseteq t\}$ has $r(\upmon_{\rho_1}(\jembed_{\rho_1}(s)))$ as minimum element, which is to say, via the induction hypothesis, that it has $r(s)$ as minimum element.  The claim then follows immediately.

  \item Assume $s \in \smng{\rho}$. For all $r \in \mmng{\rho_1}$:
  \[
    \begin{array}{rl}
    & \iembed_{\rho}(\lomon_{\rho}(s))(r) \\
    =& \iembed_{\rho_2}(\lomon_{\rho}(s)(\lomon_{\rho_1}(r))) \\
    =& \iembed_{\rho_2}(\bigcup\{\lomon_{\rho_2}(s(t)) \mid t \subseteq \iembed_{\rho_1}(\lomon_{\rho_1}(r))\}) \\
    \supseteq & \bigcup\{\iembed_{\rho_2}(\lomon_{\rho_2}(s(t))) \mid t \subseteq \iembed_{\rho_1}(\lomon_{\rho_1}(r))\} \\
    \end{array}
  \]
  since it follows from part (h) that $\iembed_{\rho_2}$ is monotone.  It follows from the induction hypothesis that $r \subseteq \iembed_{\rho_1}(\lomon_{\rho_1}(r))$ so that $\iembed_{\rho_2}(\lomon_{\rho_2}(s(r)))$ is in the given set comprehension and hence provides a lower bound to the join.  Finally, it follows from the induction hypothesis that this expression is itself no larger than $s(r)$, as required.

  \item Assume $r \in \mmng{\rho}$.  For all $s \in \smng{\rho_1}$:
  \[
    \begin{array}{rl}
      & \lomon_\rho(\iembed_{\rho}(r))(s) \\
      =& \bigcup\{\lomon_{\rho_2}(\iembed_{\rho}(r)(t)) \mid t \subseteq \iembed_{\rho_1}(s) \} \\
      =& \bigcup\{\lomon_{\rho_2}(\iembed_{\rho_2}(r(\lomon_{\rho_1}(t)))) \mid t \subseteq \iembed_{\rho_1}(s)\} \\
    \end{array}
  \]
  It then follows from the induction hypothesis that\\ $\lomon_{\rho_2}(\iembed_{\rho_2}(r(\lomon_{\rho_1}(t)))) = r(\lomon_{\rho_1}(t))$.  Since $r$ is monotone, it follows that $r(\lomon_{\rho_1}(\iembed_{\rho_1}(s)))$ is the maximum element of the set $\{r(\lomon_{\rho_1}(t)) \mid t \subseteq \iembed_{\rho_1}(s)\}$ whence, by the induction hypothesis, the join is exactly $r(s)$, as required.
\end{enumerate}
\end{proof}

\begin{lemn}[\ref{lem:galois-valuations}]
Fix a sorting $\Delta$.  For all $\alpha \in \mmng{\Delta}$, $\beta \in \smng{\Delta}$:
\begin{enumerate}[(i)]
  \item $\lomon_{\Delta}(\beta) \subseteq \alpha \equiv \beta \subseteq \iembed_{\Delta}(\alpha)$
  \item $\jembed_{\Delta}(\alpha) \subseteq \beta \equiv \alpha \subseteq \upmon_{\Delta}(\beta)$
\end{enumerate}
\end{lemn}
\begin{proof}
We only prove (i) since (ii) is completely analogous.  Let $x \in \dom(\Delta)$.  If $\Delta(x) = \iota$ then $\lomon_{\Delta}(\beta)(x) \subseteq \alpha(x)$ iff $\beta(x) = \alpha(x)$ iff $\beta(x) = \iembed_\Delta(\alpha)(x)$ iff $\beta \subseteq \iembed_\Delta(\alpha)$.  Otherwise $\Delta(x)$ is a relational sort $\rho$ and then $\lomon_\Delta(\beta)(x) \subseteq \alpha(x)$ iff $\lomon_\rho(\beta(x)) \subseteq \alpha(x)$ iff $\beta(x) \subseteq \iembed_\rho(\alpha(x))$ iff $\beta \subseteq \iembed_\Delta(\alpha)$ since it follows from Lemma \ref{lem:galois-relations} that $\lomon_\rho$ is lower adjoint to $\jembed_\rho$.
\end{proof}

\begin{lemma}\label{lem:embed-img-mono}
For all $r \in \mmng{\rho}$, $\iembed_\rho(r)$ and $\jembed_\rho(r)$ are monotone.
\end{lemma}
\begin{proof}
Immediate from the definitions since $r$ is monotone.
\end{proof}

For term $\Delta \sorts M : \sigma$ and valuations $\alpha \in \mmng{\Delta}$ (respectively $\beta \in \smng{\Delta}$) let $\alpha \restriction M$ (respectively $\beta \restriction M$) be the valuation $\alpha$  (respectively $\beta$) with domain restricted to $\fv(M)$.

\begin{lemma}\label{lem:constraint-agreement}
For all terms of the constraint language $\Delta \sorts M : \sigma \in \aterms$ and $\alpha \in \mmng{\Delta}$, $\beta \in \smng{\Delta}$:
\begin{enumerate}[(i)]
\item if $\beta \subseteq \iembed_\Delta(\alpha)$ then $\smng{M}(\beta) = \mmng{M}(\alpha)$
\item if $\alpha \subseteq \upmon_\Delta(\beta)$ then $\mmng{M}(\alpha) = \mmng{M}(\beta)$.
\end{enumerate}
\end{lemma}
\begin{proof}
Terms of the constraint language only contain variables of sort $\iota$.  Hence, it follows by definition that $\beta \restriction M = \iembed_\Delta(\alpha) \restriction M = \alpha \restriction M$ and $\alpha \restriction M = \upmon_\Delta(\beta) \restriction M = \beta \restriction M$.  The result then follows from the environment relevance property of interpretation.
\end{proof}

\begin{lemn}[\ref{lem:embed-mngs}]
Fix a sorting $\Delta$. For all goal terms $\Delta \sorts G : \rho$:
\begin{enumerate}[(i)]
\item  $\jembed_{\rho} \circ \mmng{G} \circ \upmon_{\Delta} \subseteq \smng{G}$
\item  $\lomon_{\rho} \circ \smng{G} \circ \iembed_{\Delta} \subseteq \mmng{G}$
\end{enumerate}
(with ordering given pointwise).
\end{lemn}
\begin{proof}
The proof of the first claim is by induction on the judgement $\Delta \sorts G : \rho$.
\begin{itemize}
%
\item If the judgement is $\Delta \sorts x : \rho$:
\[
  \begin{array}{rl}
           & \jembed_{\rho}(\mmng{x}(\upmon_{\Delta}(\beta))) \\
          =& \jembed_{\rho}(\upmon_{\Delta}(\beta)(x)) \\
          =& \jembed_{\rho}(\upmon_{\rho}(\beta(x))) \\
  \subseteq& \beta(x) = \smng{x}(\beta)
  \end{array}
\]
%
\item If the judgement is $\Delta \sorts HK : \rho_2$, with $\Delta \sorts H : \rho_1 \to \rho_2$ and $\Delta \sorts K : \rho_1$ then:
\[
  \begin{array}{rl}
  & \jembed_{\rho_2}(\mmng{HK}(\upmon_{\Delta}(\beta))) \\
  =& \jembed_{\rho_2}(\mmng{H}(\upmon_{\Delta}(\beta))(\mmng{K}(\upmon_{\Delta}(\beta)))) \quad(*)
  \end{array}
\]
It follows from Lemma \ref{lem:galois-relations} part (b) that:
\[
  \mmng{K}(\upmon_{\Delta}(\beta)) = \upmon_{\rho_1}(\jembed_{\rho_1}(\mmng{K}(\upmon_{\Delta}(\beta))))
\]
and hence (*) is:
\[
  \jembed_{\rho_2}(\mmng{H}(\upmon_{\Delta}(\beta))(\upmon_{\rho_1}(\jembed_{\rho_1}(\mmng{K}(\upmon_{\Delta}(\beta))))))
\]
This is, by definition:
\[
  \jembed_{\rho_1 \to \rho_2}(\mmng{H}(\upmon_{\Delta}(\beta))(\jembed_{\rho_1}(\mmng{K}(\upmon_{\Delta}(\beta))))
\]
It follows from the induction hypothesis (twice) and Lemma \ref{lem:embed-img-mono} that this is no larger than $\smng{H}(\beta)(\smng{K}(\beta)) = \smng{HK}(\beta)$.
%
\item When the judgement is $\Delta \sorts \term{H N} : \rho$ with $\Delta \sorts H : \iota \to \rho$ and $\Delta \sorts N : \iota \in \aterms$, then:
\[
  \begin{array}{rl}
    & \jembed_{\rho}(\mmng{HN}(\upmon_\Delta(\beta))) \\
    =& \jembed_{\rho}(\mmng{H}(\upmon_\Delta(\beta))(\smng{N}(\upmon_\Delta(\beta)))) \\
    =& \jembed_{\iota \to \rho}(\mmng{H}(\upmon_\Delta(\beta)))(\smng{N}(\upmon_\Delta(\beta)))
  \end{array}
\]
follows by definition.  From the induction hypothesis we obtain that this is at most:
\[
    \smng{H}(\beta)(\smng{N}(\upmon_\Delta(\beta)))
\]
and the fact that $\smng{N}(\upmon_\Delta(\beta)) = \smng{N}(\beta)$ follows from Lemma \ref{lem:constraint-agreement}.  The result then follows by definition.
%
\item If $G$ is an abstraction $\abs{x}{H}$ then $\rho$ is either of the form $\iota \to \rho'$ or $\rho_1 \to \rho_2$.  Both cases are similar, so we consider the latter only. Then let $s \in \smng{\rho_1}$.  It follows that:
\[
  \begin{array}{rl}
    & \jembed_{\rho}(\mmng{\abs{x}{H}}(\upmon_{\Delta}(\beta)))(s) \\
    =& \jembed_{\rho_2}(\mmng{\abs{x}{H}}(\upmon_{\Delta}(\beta))(\upmon_{\rho_1}(s))) \\
    =& \jembed_{\rho_2}(\mmng{H}(\upmon_{\Delta}(\beta)[x \mapsto \upmon_{\rho_1}(s)])) \\
    =& \jembed_{\rho_2}(\mmng{H}(\upmon_{\Delta,x:\rho_1}(\beta[x \mapsto s])))
  \end{array}
\]
by definition.  From the induction hypothesis, we can conclude that this is no larger than $\smng{H}(\beta[x \mapsto s])$ which is just $\smng{\abs{x}{H}}(\beta)(s)$, as required.

\item If the judgement is $\Delta \sorts \phi : o$ then:
\[
  \jembed_{\boolsort}(\mmng{\phi}(\upmon_{\Delta}(\beta))) = \mmng{\phi}(\upmon_{\Delta}(\beta))
\]
Since $\phi$ is, in particular, a term of the constraint language, it follows from Lemma \ref{lem:constraint-agreement} that this is the same as $\mmng{\phi}(\beta)$.  Finally, by definition, $\mmng{\phi}(\beta) = \smng{\phi}(\beta)$.

\item If the judgement is $\Delta \sorts c: o \to o \to o$ for one of the binary positive logical connectives, then it follows that:
\[
  \jembed_{o \to o \to o}(\mmng{c}(\upmon_{\Delta}(\beta))) = \mmng{c}(\upmon_{\Delta}(\beta))
\]
since $\jembed_{\rho}$ is the identity when $\rho$ is first-order and $\mmng{c}(\upmon_{\Delta}(\beta)) = \smng{c}(\beta)$ since the meaning of $c$ is independent of the valuation and the standard and monotone interpretations of these constants are the same.

\item If the judgement is $\Delta \sorts \exists_\iota : (\iota \to \boolsort) \to \boolsort$, then let $s \in \smng{\iota \to \boolsort}$.  It follows that:
\[
  \begin{array}{rl}
  & \jembed_{\rho}(\mmng{\exists_\iota}(\upmon_{\Delta}(\beta)))(s) \\
  =& \jembed_{\boolsort}(\mmng{\exists_\iota}(\upmon_{\Delta}(\beta))(\upmon_{\iota \to \boolsort}(s))) \\
  =& \mmng{\exists_\iota}(\upmon_{\Delta}(\beta))(s) \\
  \end{array}
\]
since $\iembed_{\rho}$ and $\lomon_{\rho}$ act as the identity when $\rho$ is first-order.  Finally, it follows from the definition of $\mmng{\exists_\iota}$ that this last expression is exactly $\smng{\exists_\iota}(\beta)(s)$, as required.

\item If $G$ is $\exists_\rho : (\rho \to \boolsort) \to \boolsort$, then let $s \in \smng{\rho}$.
It follows that:
\[
  \begin{array}{rl}
    & \jembed_{(\rho \to \boolsort) \to \boolsort}(\mmng{\exists_\rho}(\upmon_{\Delta}(\beta)))(s) \\
    =& \jembed_{\boolsort}(\mmng{\exists_\rho}(\upmon_{\Delta}(\beta))(\upmon_{\rho \to \boolsort}(s))) \\
    =& \mmng{\exists_\rho}(\upmon_{\Delta}(\beta))(\upmon_{\rho \to \boolsort}(s)) \\
  \end{array}
\]
by definition.  Assume that this expression is identical to $1$.  Then there is some $r \in \mmng{\rho}$ such that $\upmon_{\rho \to \boolsort}(s)(r) = 1$, which is to say that $\bigcap\{\upmon_{\boolsort}(s(t)) \mid \jembed_\rho(r) \subseteq t\} = 1$.  Necessarily then, for any $t$ no smaller than $\jembed_\rho(r)$, $\upmon_{o}(s(t)) = s(t) = 1$.  Hence, in particular $s(\jembed_\rho(r)) = 1$ whence $\smng{\exists_\rho}(\beta)(s) = 1$.
\end{itemize}
For the second claim, we prove the stronger statement: \\
For all $\alpha \in \mmng{\Delta}, \beta \in \smng{\Delta}$:
\[
  \beta \subseteq \iembed_\Delta(\alpha) \quad\text{implies}\quad \lomon_\rho(\smng{G}(\beta)) \subseteq \mmng{G}(\alpha)
\]
by induction on $\Delta \sorts G : \rho$.
\begin{itemize}
  %
  \item If the judgement is $\Delta \sorts x : \rho$, assume $\beta \subseteq \iembed_\Delta(\alpha)$.  Then:
  \[
    \lomon_{\rho}(\smng{G}(\beta)) = \lomon_\rho(\beta(x)) \subseteq \lomon_\rho(\iembed_\Delta(\alpha)(x))
  \]
  by assumption and the monotonicity of $\lomon_\rho$.  Then:
  \[
    \lomon_\rho(\iembed_\Delta(\alpha(x))) = \alpha(x) = \mmng{G}(\alpha)
  \]
  by Lemma \ref{lem:galois-relations} part (iv).
  %
  \item If the judgement is $\Delta \sorts \term{H K} : \rho_2$ and $\Delta \sorts H : \rho_1 \to \rho_2$ and $\Delta \sorts K : \rho_1$ then assume $\beta \subseteq \iembed_\Delta(\alpha)$.  We first observe that $\lomon_{\rho_2}(\smng{G}(\beta)) = \lomon_{\rho_2}(\smng{H}(\beta)(\smng{K}(\beta)))$ by definition.  We claim that:
  \[
    \lomon_{\rho_2}(\smng{H}(\beta)(\smng{K}(\beta))) \subseteq \lomon_{\rho_1 \to \rho_2}(\smng{H}(\beta))(\lomon_{\rho_2}(\smng{K}(\beta)))
  \]
  To see this, note that the latter expression is, by definition:
  \[
    \bigcup\{ \lomon_{\rho_2}(\smng{H}(\beta)(t)) \mid t \subseteq \iembed_{\rho_1}(\lomon_{\rho_1}(\smng{K}(\beta)))\}
  \]
  Since, by Lemma \ref{lem:galois-relations} part (iii), $\smng{K}(\beta)$ is one such $t$, the set comprehension contains, and hence the join is bounded below by, $\lomon_{\rho_2}(\smng{H}(\beta)(\smng{K}(\beta)))$, thus proving the claim.  Next we observe that
  \[
    \lomon_{\rho_1 \to \rho_2}(\smng{H}(\beta))(\lomon_{\rho_2}(\smng{K}(\beta))) \subseteq \mmng{H}(\alpha)(\lomon_{\rho_2}(\smng{K}(\beta)))
  \]
  follows from the induction hypothesis.  Finally, since $\mmng{H}(\alpha)$ is monotone, it follows from the induction hypothesis that:
  \[
    \mmng{H}(\alpha)(\lomon_{\rho_2}(\smng{K}(\beta))) \subseteq \mmng{H}(\alpha)(\mmng{K}(\alpha))
  \]
  and this is exactly $\mmng{G}(\alpha)$.
  %
  \item If the judgement is $\Delta \sorts \term{H N} : \rho$ and $\Delta \sorts H : \iota \to \rho$ and $\Delta \sorts N : \iota$, assume $\beta \subseteq \iembed_\Delta(\alpha)$.  Then
  \[
    \begin{array}{rl}
    &\lomon_{\rho}(\smng{G}(\beta)) \\
    =& \lomon_{\rho}(\smng{H}(\beta)(\smng{N}(\beta))) \\
    =& \lomon_{\iota \to \rho}(\smng{H}(\beta))(\smng{N}(\beta)) \\
    \subseteq& \mmng{H}(\alpha)(\smng{N}(\beta))
    \end{array}
  \]
  follows by definition and the induction hypothesis.  Since $\beta \subseteq \iembed_\Delta(\alpha)$ and $N$ is a term of the constraint language, it follows from Lemma \ref{lem:constraint-agreement} that $\smng{N}(\beta) = \smng{N}(\alpha)$ as required.
  %
  \item If the judgement is $\Delta \sorts \abs{x\!\!:\!\!\iota}{H} : \iota \to \rho$ then assume $\beta \subseteq \iembed_\Delta(\alpha)$.  For all $n \in \mmng{\iota}$:
  \[
    \lomon_{\iota \to \rho}(\smng{G}(\beta))(n) = \lomon_\rho(\smng{G}(\beta)(n)) = \lomon_\rho(\smng{H}(\beta[x \mapsto n]))
  \]
  Since $\beta[x \mapsto n] \subseteq \iembed_\Delta(\alpha)[x \mapsto n] = \iembed_{\Delta,x:\iota}(\alpha[x \mapsto n])$, it follows from the induction hypothesis that:
  \[
    \lomon_\rho(\smng{H}(\beta[x \mapsto n])) = \mmng{H}(\alpha[x \mapsto n])
  \]
  and, by definition, $\mmng{H}(\alpha[x \mapsto n]) = \mmng{G}(\alpha)(n)$.
  %
  \item If the judgement is $\Delta \sorts \abs{x\!\!:\!\!\rho_1}{H} : \rho_2$, then assume $\beta \subseteq \iembed_\Delta(\alpha)$.  For all $r \in \mmng{\rho_1}$:
  \[
    \begin{array}{rl}
       & \lomon_{\rho_1 \to \rho_2}(\smng{G}(\beta))(r) \\
      =& \bigcup \{\lomon_{\rho_2}(\smng{G}(\beta)(t)) \mid t \subseteq \iembed_{\rho_1}(r)\} \\
      =& \bigcup \{\lomon_{\rho_2}(\smng{H}(\beta[x \mapsto t])) \mid t \subseteq \iembed_{\rho_1}(r)\}
    \end{array}
  \]
  follows by definition.  Notice that, for all such $t$, $\beta[x \mapsto t] \subseteq \iembed_{\Delta,x:\rho_1}(\alpha[x \mapsto r])$ since $\beta \subseteq \iembed_\Delta(\alpha)$ and $t \subseteq \iembed_{\rho_1}(r)$, $x \notin \dom(\Delta)$.  Therefore, it follows from the induction hypothesis that every element of the set comprehension is bounded above by
  $\mmng{H}(\alpha[x \mapsto r])$
  and hence the whole join is bounded above by the same relation.
  The result then follows by definition since $\mmng{H}(\alpha[x \mapsto r]) = \mmng{G}(\alpha)(r)$.
  %
  \item When the judgement is of shape $\Delta \sorts c : \boolsort \to \boolsort \to \boolsort$ for $c$ either $\vee$ or $\wedge$, assume $\beta \subseteq \iembed_\Delta(\alpha)$.  Since $c$ is first order, it follows that $\lomon_{\boolsort \to \boolsort \to \boolsort}(\smng{c}(\beta)) = \smng{c}(\beta)$ and since the meaning of $c$ is independent of the environment and identical in the standard and monotone interpretations,
  $\smng{c}(\beta) = \mmng{c}(\alpha)$.
  %
  \item When the judgement is of shape $\Delta \sorts \phi : \boolsort$ for a constraint formula $\phi$, assume $\beta \subseteq \iembed_\Delta(\alpha)$.  By definition $\lomon_\boolsort(\smng{\phi}(\beta)) = \smng{\phi}(\beta)$.  Since $\phi$ is, in particular, a term of the constraint language, it follows from Lemma \ref{lem:constraint-agreement} that $\smng{\phi}(\beta) = \mmng{\phi}(\alpha)$.
  %
  \item When the judgement is of shape $\Delta \sorts \exists_\iota : (\iota \to \boolsort) \to \boolsort$, it follows by definition that, for all $r \in \mmng{\iota \to \boolsort}$:
  \[
    \begin{array}{rl}
       & \lomon_{(\iota \to \boolsort) \to \boolsort}(\smng{\exists_\iota}(\beta))(r) \\
      =& \bigcup \{ \lomon_\boolsort(\smng{\exists_\iota}(\beta)(t)) \mid t \subseteq \iembed_{\iota \to \boolsort}(r) \} \\
      =& \bigcup \{ \smng{\exists_\iota}(\beta)(t) \mid t \subseteq r \}
    \end{array}
  \]
  We claim that this last expression is no larger than $\mmng{\exists_\iota}(\alpha)(r)$.  To see this, observe that if this last expression is $1$, then it must be that there is some $t \in \smng{\iota \to \boolsort}$ such that $t \subseteq r$ and some $n \in \smng{\iota}$ such that $t(n) = 1$.  Therefore, also there is some $n \in \mmng{\iota} = \smng{\iota}$ such that $r(n) = 1$.  Hence $\mmng{\exists_\iota}(\alpha)(r) = 1$ as required.
  %
  \item When the judgement has shape $\Delta \sorts \exists_\rho : (\rho \to \boolsort) \to \boolsort$, it follows by definition that, for all $r \in \mmng{\rho \to \boolsort}$:
  \[
    \begin{array}{rl}
       & \lomon_{(\rho \to \boolsort) \to \boolsort}(\smng{\exists_\rho}(\beta))(r) \\
      =& \bigcup \{ \lomon_\boolsort(\smng{\exists_\rho}(\beta)(t)) \mid t \subseteq \iembed_{\rho \to \boolsort}(r) \} \\
      =& \bigcup \{ \smng{\exists_\rho}(\beta)(t) \mid t \subseteq \iembed_{\rho \to \boolsort}(r) \}
    \end{array}
  \]
  We claim that this last expression is no larger than $\mmng{\exists_\rho}(\alpha)(r)$.  To see this, observe that if this last expression is $1$, then it must be that there is some $t \subseteq \iembed_{\rho \to \boolsort}(r)$ and $s \in \smng{\rho}$ such that $t(s) = 1$.  But then, $\iembed_{\rho \to \boolsort}(r)(s) = 1$.  By definition, $\iembed_{\rho \to \boolsort}(r)(s) = \iembed_\boolsort(r(\lomon_\rho(s)))$, so $r(\lomon_\rho(s)) = 1$.  Hence $\lomon_\rho(s) \in \mmng{\rho}$ is the required witness to the fact that $\mmng{\exists_\rho}(\alpha)(r) = 1$.
\end{itemize}
\end{proof}


==> apx-opsem.tex <==
%

\section{Operational Semantics}\label{sec:apx-opsem}

Given a program $p$, we define a small-step operational semantics whose normal forms are constraint formulas.

\begin{prooftree}
\AxiomC{}
\LeftLabel{\EBeta}
\UnaryInfC{$(\abs{x}{s})t \stepsto s[t/x]$}
\end{prooftree}
\begin{prooftree}
\AxiomC{}
\LeftLabel{\EDelta}
\RightLabel{$p(x) = s$}
\UnaryInfC{$x \stepsto s$}
\end{prooftree}
\begin{prooftree}
\AxiomC{$s \stepsto s'$}
\LeftLabel{\EAppL}
\UnaryInfC{$\term{s t} \stepsto \term{s' t}$}
\end{prooftree}
\begin{prooftree}
\AxiomC{$t \stepsto t'$}
\LeftLabel{\EAppR}
\UnaryInfC{$\term{s t} \stepsto \term{s' t}$}
\end{prooftree}
\begin{prooftree}
\AxiomC{$s \stepsto s'$}
\LeftLabel{\EAbs}
\UnaryInfC{$\abs{x}{s} \stepsto \abs{x}{s'}$}
\end{prooftree}

%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%

%
%



%
%
%

%
%

==> apx-ty-guards.tex <==
%

\section{Proofs from Section 6}

\begin{lemma}\label{lem:upper-adj-conv}
Let $\Delta \sorts T :: \rho$ be a type and $\alpha \in \smng{\Delta}$ a first-order valuation. Then:
\begin{enumerate}[(i)]
\item $\upmon_\rho(\rsmng{T}(\alpha)) = \rmmng{T}(\alpha)$
\item and $\iembed_\rho(\rmmng{T}(\alpha)) = \rsmng{T}(\alpha)$.
\end{enumerate}
\end{lemma}
\begin{proof}
The proof is by induction on $\Delta \sorts T :: \rho$.
\begin{itemize}
\item When the judgement is $\Delta \sorts \boolty{\phi} :: \boolsort$, the result is immediate by definition.
\item When the judgement is $\Delta \sorts \dto{x}{\iota}{T} :: \iota \to \rho$, for all $n \in A_\iota$:
\[
  \upmon_{\iota\to\rho}(\rsmng{\dto{x}{\iota}{T}}(\alpha))(n) = \upmon_\rho(\rsmng{\dto{x}{\iota}{T}}(\alpha)(n)) = \upmon_\rho(\rsmng{T}(\alpha[x \mapsto n]))
\]
and this last expression is exactly $\rmmng{T}(\alpha[x \mapsto n]) = \rmmng{x}{\iota}{T}(\alpha)(n)$ by the induction hypothesis, thus demonstrating (i).  Point (ii) follows analogously.
\item When the judgement is $\Delta \sorts T_1 \to T_2 :: \rho_1 \to \rho_2$, for all $r \in \mmng{\rho_1}$:
\[
  \upmon_{\rho_1 \to \rho_2}(\rsmng{T_1 \to T_2}(\alpha))(r) = \bigcap\{\upmon_{\rho_2}(\rsmng{T_1 \to T_2}(\alpha)(t)) \mid \jembed(r) \subseteq t\}
\]
Since, by Lemma \ref{lem:ty-interp-mono}, $\rsmng{T_1 \to T_2}(\alpha)$ is monotone, it follows that the set comprehension has a minimum element, $\upmon_{\rho_2}(\rsmng{T_1 \to T_2}(\alpha)(\jembed(r))$, and so this element is its meet.
Observe that $r \subseteq \rmmng{T_1}(\alpha)$ iff $\jembed_{\rho_1}(r) \subseteq \rsmng{T_1}(\alpha)$.
To see this, notice that it follows from the induction hypothesis that $r \subseteq \rmmng{T_1}(\alpha)$ iff $r \subseteq \upmon_{\rho_1}(\smng{T_1}(\alpha))$ and since, by Lemma \ref{lem:galois-relations}, $\upmon_{\rho_1}$ is upper adjoint to $\jembed_{\rho_1}$, this latter expression is equivalent to $\jembed_{\rho_1}(r) \subseteq \smng{T_1}(\alpha)$.
We now distinguish two cases.
\begin{itemize}
  \item In case $r \subseteq \rmmng{T_1}(\alpha)$, $\rmmng{T_1 \to T_2}(\alpha) = \rmmng{T_2}(\alpha)$.  It follows from the observation that, therefore, $\upmon_{\rho_2}(\rsmng{T_1 \to T_2}(\alpha)(\jembed_{\rho_1}(r)) = \upmon_{\rho_2}(\rsmng{T_2}(\alpha))$ and the result follows from the induction hypothesis.
  \item In case $r \not\subseteq \rmmng{T_1}(\alpha)$, $\rmmng{T_1 \to T_2}(\alpha) = \top_{\rho_2}$.  It follows from the observation that also, therefore, $\upmon_{\rho_2}(\rsmng{T_1 \to T_2}(\alpha)(\jembed_{\rho_1}(r)) = \top_{\rho_2}$.
\end{itemize}
This demonstrates point (i).
For point (ii), $\iembed_{\rho_1 \to \rho_2}(\rmmng{T_1 \to T_2}(\alpha))(r) = \iembed_{\rho_2}(\rmmng{T_1 \to T_2}(\alpha)(\lomon_{\rho_1}(r)))$ by definition.  Observe that:
\[
  s \subseteq \rsmng{T_1}(\alpha) \quad\textit{iff}\quad r \subseteq \iembed_{\rho_1}(\rmmng{T_1}(\alpha)) \quad\textit{iff}\quad \lomon_{\rho_1}(r) \subseteq \rmmng{T_1}(\alpha)
\]
follows from the induction hypothesis and the fact that, by Lemma \ref{lem:galois-relations}, $\lomon_{\rho_1}$ is lower adjoint to $\iembed_{\rho_1}$.  The result then follows by case analysis as for point (i).
\end{itemize}
\end{proof}

\begin{thmn}[\ref{thm:ty-guard-red-s-to-m}]
Type-guarded, higher-order constrained Horn clause problem $\abra{\Delta,D,G}$ is solvable iff type-guarded, monotone logic safety problem $\abra{\Delta,P_D,G}$ is solvable.
\end{thmn}
\begin{proof}
Considering the two cases for relational existentials $\exists_{\rho}$ in the proof of Lemma \ref{lem:embed-mngs}, to additionally take account of type-guarded existentials we need only show that:
\begin{itemize}
\item Whenever there is a witness $r \in \mmng{T}$, also $\jembed_{\rho}(r) \in \smng{T}$
\item and whenever there is a witness $s \in \smng{T}$ for $\beta \subseteq \iembed_\Delta(\alpha)$, also $\lomon_\rho(s) \in \mmng{T}$.
\end{itemize}
This follows from Lemmas \ref{lem:galois-relations}, \ref{lem:types-are-pideals} and \ref{lem:upper-adj-conv}.  If $r \in \mmng{T}$ then $r \subseteq \rmmng{T}$ and hence $r \subseteq \upmon_\rho(\rsmng{T})$.  Since $\upmon_\rho$ is upper adjoint to $\jembed_\rho$, therefore $\jembed_\rho(r) \subseteq \rsmng{T}$, i.e. $\jembed_\rho(r) \in \smng{T}$.
Similarly, if $\beta \subseteq \iembed_\Delta(\alpha)$ and $s \in \smng{T}$, then $s \subseteq \rsmng{T}$ and $s \subseteq \iembed_\rho(\rmmng{T})$.  Since $\iembed_\rho$ is upper adjoint to $\lomon_\rho$, therefore $\lomon_\rho(s) \subseteq \rmmng{T}$, i.e. $\lomon_\rho(s) \in \mmng{T}$.
\end{proof}

\begin{lemn}[\ref{lem:G-defns}]
For any closed type $\sorts T :: \rho$:
\begin{enumerate}[(i)]
  \item The goal term $\com(T)$ is a $G$-definition of the class $\{r \in \mmng{\rho} \mid r \notin \mmng{T}(\emptyset)\}$.
  \item The goal term $\lar(\falsetm)(T)$ is a $G$-definition of the relation $\rmmng{T}(\emptyset)$.
\end{enumerate}
\end{lemn}
\begin{proof}
We generalise the statement, proving for all $\Delta \sorts T :: \rho$, $\alpha \in \mmng{\Delta}$ and goal formulas $\Delta \sorts G : \boolsort$: $\mmng{\com(T)}(\alpha) = \{r \in \mmng{\rho} \mid r \notin \mmng{T}(\alpha)\}$ and, for all $\vv{d}$ of the appropriate sorts: $\mmng{\lar(G)(T)}(\alpha)(\vv{d}) = 1$ iff $\mmng{G}(\alpha)$ = 1 or $\rmmng{T}(\alpha)(\vv{d}) = 1$.
The proof is by induction on $\Delta \sorts T :: \rho$.
\begin{itemize}
  \item If the judgement is of shape $\Delta \sorts \boolty{\phi} :: o$ then we reason as follows.
  \begin{enumerate}[(i)]

    \item For all $b \in \mathbbm{2}$:
    \[
      \mmng{\com(T)}(\alpha)(b) = \mmng{x \wedge \neg\phi}(\alpha[x \mapsto b])
    \]
    This latter expression evaluates to $1$ iff $\alpha[x \mapsto b] \not\models x \implies \phi$ (by the variable convention we assume that $x$ does not occur in $\phi$).
    It follows from Lemma \ref{lem:boolty-meaning} that this is the case iff $\mmng{x}(\alpha[x \mapsto b]) = b \notin \mmng{T}(\alpha[x \mapsto b]) = \mmng{T}(\alpha)$.

    \item Also, $\mmng{\lar(G)(T)}(\alpha) = \mmng{G \vee \phi}(\alpha) = \orfn(\mmng{G}(\alpha))(\mmng{\phi}(\alpha))$.  This latter expression denotes $1$ iff $\mmng{G}(\alpha) = 1$ or $\mmng{\phi}(\alpha) = 1$.
  \end{enumerate}

  \item If the judgement is of shape $\Delta \sorts \dto{x}{\iota}{T'} :: \iota \to \rho$ then we reason as follows.
  \begin{enumerate}[(i)]
    \item For all $r \in \mmng{\iota \to \rho}$:
    \[
      \mmng{\com(T)}(\alpha)(r) = \mmng{\exists x\!\!:\!\!\iota.\,\com(T')(z\,x)}(\alpha[z \mapsto r])
    \]
    This latter expression denotes $1$ iff there is some $n \in A_\iota$ such that $\mmng{\com(T')(x\,y)}(\alpha[z \mapsto r][x \mapsto n]) = 1$ and this is true iff there is some $n$ such that $\mmng{\com(T')}(\alpha[x \mapsto n])(r(n)) = 1$.  It follows from the induction hypothesis that this is true iff there is some $n$ such that $r(n) \notin \mmng{T'}(\alpha[x \mapsto n])$.  This is exactly $r \notin \mmng{\dto{x}{\iota}{T'}}(\alpha)$.

    \item For all $n \in A_\iota$ and $\vv{d}$:
    \[
      \mmng{\lar(G)(T)}(\alpha)(n)(\vv{d}) = \mmng{\lar(G)(T')}(\alpha[x \mapsto n])(\vv{d})
    \]
    It follows from the induction hypothesis that this denotes $1$ iff either $\mmng{G}(\alpha[x \mapsto n]) = 1$ or $\rmmng{T'}(\alpha[x \mapsto n])(\vv{d}) = 1$.  We may assume, by the variable convention, that $x$ does not occur in $G$.  This latter expression denotes $1$ iff $\rmmng{\dto{x}{\iota}{T'}}(\alpha)$ by definition.
  \end{enumerate}

  \item If the judgement is of shape $\Delta \sorts T_1 \to T_2 :: \rho_1 \to \rho_2$ then we reason as follows.
  \begin{enumerate}[(i)]
    \item For all $r \in \mmng{\rho_1 \to \rho_2}$:
    \[
      \mmng{\com(T)}(\alpha)(r) = \mmng{\com(T_2)(x\,\lar(\falsetm)(T_1))}(\alpha[x \mapsto r])
    \]
    This latter expression is true iff $\mmng{\com(T_2)}(\alpha)(r(\mmng{\lar(\falsetm)(T_1)}(\alpha))) = 1$.  It follows from the induction hypothesis, part (ii), that this is the case iff $\mmng{\com(T_2)}(\alpha)(r(\rmmng{T_1}(\alpha))) = 1$.  By the monotonicity of the operator and the fact that $\rmmng{T_1}(\alpha)$ is the largest element of $\mmng{T_1}(\alpha)$ (Lemma \ref{lem:types-are-pideals}), this is true iff there is some $s \in \mmng{T_1}(\alpha)$ such that $\mmng{\com(T_2)}(\alpha)(r(s)) = 1$.  It follows from the induction hypothesis, part (i), that this is true iff there is some $s \in \mmng{T_1}(\alpha)$ such that $r(s) \notin \mmng{T_2}(\alpha)$, which is exactly $r \notin \mmng{T_1 \to T_2}(\alpha)$.

    \item Fix $r \in \mmng{\rho_1}(\alpha)$ and $\vv{d}$ appropriate to the argument sorts of $\rho_2$.  Then:
    \[
      \mmng{\lar(G)(T)}(\alpha)(r)(\vv{d}) = \mmng{\lar(G \vee \com(T_1)\,x)(T_2)}(\alpha[x \mapsto r])(\vv{d})
    \]
    It follows from the induction hypothesis, part (ii), that this expression denotes $1$ iff (P1) $\mmng{G \vee \com(T_1)\,x}(\alpha[x \mapsto r]) = 1$ or (P2) $\rmmng{T_2}(\alpha)(\vv{d}) = 1$.
    It follows that this first possibility (P1) is true iff $\mmng{G}(\alpha) = 1$ or $\mmng{\com(T_1)}(\alpha)(r) = 1$.
    It follows from the induction hypothesis, part (i), that $\mmng{\com(T_1)}(\alpha)(r) = 1$ iff $r \notin \mmng{T_1}(\alpha)$.
    Consequently, (P1) or (P2) iff $\mmng{G}(\alpha) = 1$ or (Q1) $r \notin \mmng{T_1}(\alpha)$ or (Q2) $\rmmng{T_2}(\alpha)(\vv{d}) = 1$.
    We claim that (Q1) or (Q2) iff $\rmmng{T}(\alpha)(r)(\vv{d}) = 1$.
    In the backward direction, assume that (Q1) does not hold.  Then, by Lemma \ref{lem:types-are-pideals}, $r \subseteq \rmmng{T_1}(\alpha)$ and $\rmmng{T}(\alpha)(r)(\vv{d}) = 1$ implies $\rmmng{T_2}(\alpha)(r)(\vv{d}) = 1$ which is (Q2).
    In the forward direction we analyse the two cases.
    In case (Q1), by Lemma \ref{lem:types-are-pideals}, $r \not\subseteq \rmmng{T_1}(\alpha)$.  Then $\rmmng{T}(\alpha)(r)(\vv{d}) = \top_{\rho_2}(r)(\vv{d}) = 1$ by definition.
    Otherwise we assume (Q2) and not (Q1).
    Then, by Lemma \ref{lem:types-are-pideals}, $r \subseteq \rmmng{T_1}(\alpha)$, so $\rmmng{T_2}(\alpha)(\vv{d}) = 1$ implies $\rmmng{T}(\alpha)(r)(\vv{d}) = 1$ by definition.
  \end{enumerate}
\end{itemize}
\end{proof}

\begin{thmn}[\ref{thm:ty-guard-elim-final}]
Type guarded, higher-order constrained Horn clause problem $\abra{\Delta,D,G}$ is solvable iff monotone logic program safety problem $\abra{\Delta,\mathsf{Elim}(P_D),\mathsf{Elim}(G)}$ is solvable.
\end{thmn}
\begin{proof}
It is possible to show by induction that, for type-guarded goal term $G$, $\mmng{G} = \mmng{\mathsf{Elim}(G)}$.  We consider only the case in which $G$ has shape $\exists x\!\!:\!\!T.\,H$, since the others are straightforward.  So, assume that $\mmng{H} = \mmng{\mathsf{Elim}(H)}$.  Then it follows from a property of substitution and Lemma \ref{lem:G-defns} that:
\[
  \mmng{\mathsf{Elim}(\exists x\!:\!T.\,H)}(\alpha) = \mmng{H}(\alpha[x \mapsto \mmng{\lar(\falsetm)(T)}(\emptyset)]) = \mmng{H}(\alpha[x \mapsto \rmmng{T}(\emptyset)])
\]
Recall that $\mmng{H}$ is monotone and that, by Lemma \ref{lem:types-are-pideals}, $\rmmng{T}(\emptyset)$ is the largest element of $\mmng{T}(\emptyset)$.  Hence, $\mmng{H}(\alpha[x \mapsto \rmmng{T}(\emptyset)]) = 1$ iff there is some $r \in \mmng{T}(\emptyset)$ such that $\mmng{H}(\alpha[x \mapsto r]) = 1$.  By definition, this is true iff $\mmng{\exists x\!:\!T.\,H}(\alpha) = 1$.  Hence $\mmng{\mathsf{Elim}(\exists x\!:\!T.\,H)} = \mmng{\exists x\!:\!T.\,H}$, as required.

Consequently, for all $x \in \dom(\Delta)$, $\mfunc_{P_D}(\alpha)(x) = \mmng{P(x)}(\alpha) = \mmng{\mathsf{Elim}(P(x))} = \mfunc_{\mathsf{Elim}(P)}(\alpha)(x)$ and, therefore, $\mfunc_{P}$ and $\mfunc_{\mathsf{Elim}(P)}$ have the same prefix points. Hence, type-guarded monotone problem $\abra{\Delta,P,G}$ is solvable iff monotone problem $\abra{\Delta,\mathsf{Elim}(P),\mathsf{Elim}(G)}$ is solvable.  The result then follows from Theorem \ref{thm:ty-guard-red-s-to-m}.
\end{proof}

